Automated Update of Android Deprecated API Usages with Large Language Models

Android apps rely on application programming interfaces (APIs) to access various functionalities of Android devices. These APIs however are regularly updated to incorporate new features while the old APIs get deprecated. Even though the importance of updating deprecated API usages with the recommended replacement APIs has been widely recognized, it is non-trivial to update the deprecated API usages. Therefore, the usages of deprecated APIs linger in Android apps and cause compatibility issues in practice. This paper introduces GUPPY, an automated approach that utilizes large language models (LLMs) to update Android deprecated API usages. By employing carefully crafted prompts, GUPPY leverages GPT-4, one of the most powerful LLMs, to update deprecated-API usages, ensuring compatibility in both the old and new API levels. Additionally, GUPPY uses GPT-4 to generate tests, identify incorrect updates, and refine the API usage through an iterative process until the tests pass or a specified limit is reached. Our evaluation, conducted on 360 benchmark API usages from 20 deprecated APIs and an additional 156 deprecated API usages from the latest API levels 33 and 34, demonstrates GUPPY's advantages over the state-of-the-art techniques.

==> sections/abstract.tex <==
\begin{abstract}
Android apps rely on application programming interfaces (APIs) to
access various functionalities of Android devices.
%during app development. 
These APIs however are regularly updated to incorporate new features while the old APIs get deprecated. Even though the importance of updating
deprecated API usages with the recommended replacement APIs has been widely recognized, it is non-trivial to update the
deprecated API usages. Therefore,  the usages of deprecated APIs linger in Android apps and cause compatibility issues in practice.
%many Android apps still use deprecated APIs, resulting in compatibility issues in practice. 
This paper introduces \tool, an automated approach that utilizes large language models (LLMs) to update Android deprecated API usages. By employing
carefully crafted prompts, \tool\ leverages GPT-4, one of the
most powerful LLMs, to update deprecated-API usages, ensuring
compatibility in both the old and new API levels. Additionally, \tool\
uses GPT-4 to generate tests, identify incorrect updates, and refine
the API usage through an iterative process until the tests pass or a
specified limit is reached. Our evaluation, conducted on 360
benchmark API usages from 20 deprecated APIs and an additional 156
deprecated API usages from the latest API levels 33 and 34,
demonstrates \tool's advantages over the state-of-the-art techniques.

%Developers rely on Android application programming interfaces (APIs) to access and use the various functionalities of Android devices during app development. With the continuous evolution of the Android operating system, these APIs are regularly updated to incorporate new features and deprecate older ones. Despite these updates, many Android apps still use deprecated APIs, which results in compatibility issues. While the importance of updating deprecated API usages with the recommended replacement APIs has been widely recognized, it is non-trivial in practice to update the deprecated API usages.

%This paper introduces \tool\ that utilizes large language models (LLMs) to update deprecated API usages in Android apps. By employing carefully crafted prompts, \tool\ leverages GPT-4, one of the most powerful LLMs, to update deprecated APIs, ensuring compatibility in both old and new API levels. Additionally, \tool\ uses GPT-4 to generate tests, identify incorrect updates, and refine the API usage through an iterative process until the tests pass or a specified limit is reached.

%Our evaluation, conducted on 360 benchmark API usages from 20 deprecated APIs and an additional 156 deprecated API usages from the latest API levels 33 and 34, demonstrates \tool’s significant advantages over current state-of-the-art techniques.
\end{abstract}




==> sections/implications.tex <==
\section{Implications} \label{implications}
Based on the usage of the large language model, here are some implications for researchers and developers that can be used in \bin{ the future}:
\begin{itemize}
    \item Prompt Construction is Key: Developers utilizing AI-driven code generators like GPT-4 should invest time in meticulously crafting prompts. The quality and specificity of the prompt directly influence the output quality.
    \item Testing Versatility: Robolectric's ability to test across multiple API levels offers a unique advantage for researchers and developers alike. It underscores the importance of employing versatile testing frameworks, especially in the dynamic landscape of API evolutions.
    \item Addressing Dependencies: The evaluation illuminated challenges related to code dependencies, especially concerning different objects or activities. This reiterates the importance for developers to consider context-aware testing, particularly when managing intricate dependencies.
    \item Iterative Process for Enhancements: While zero-shot approaches present great promise, they also come with limitations. Researchers might consider iterative or multi-shot approaches to refine and enhance results further.
    \item Critical Evaluation of AI-Generated Tests: The instance where a test should have ideally failed, but didn't, suggests that while AI can generate tests, human judgment remains paramount. Developers should critically assess and possibly fine-tune AI-generated tests to ensure they're catching all potential issues.
    \item Ongoing Training for AI Models: Given the evolving nature of software, regular training and updates for models like GPT-4 are essential. Researchers could consider collaborative frameworks where real-world usage and feedback iteratively refine AI models.
\end{itemize}

These implications can guide both the academic community and industry practitioners in the utilization, development, and enhancement of AI tools and methodologies in the realm of software engineering.

==> sections/prompt.tex <==
\section{Prompt Engineering} \label{sec:prompt}





==> tables/apps.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{Selected Android apps for the study}
\label{tab:apps}
\centering
\scalebox{1.00}{
\begin{tabular}{|l|c|c|c|c|c|c|}
	\hline
	App name                & Category                  & Installs    & First Release & Version & \# Tags & \# Commits \\ \hline
	AmazeFileManager        & Tools                     & 1,000,000+  & Nov 11, 2014  & 3.3.4   & 52      & 4611       \\ \hline
	AnkiDroid               & Education                 & 5,000,000+  & May 31, 2009  & 2.8.4   & 977     & 12435      \\ \hline
	Budget Watch            & Finance                   & 1,000+      & Feb 7, 2016   & 0.21.5  & 29      & 477        \\ \hline
	Chibe                   & Tools                     & -           & Nov 27, 2016  & 1.2.1   & 4       & 144        \\ \hline
	CineLog                 & Video Players \& Editors  & 1,000+      & Nov 5, 2018   & 0.2.1   & 16      & 349        \\ \hline
	Connectbot              & Communication             & 1,000,000+  & Oct 1, 2008   & 1.9.5   & 454     & 1920       \\ \hline
	DNS66                   & Tools                     & -           & Oct 19, 2016  & 0.6.1   & 29      & 359        \\ \hline
	Download Navi           & Tools                     & 10,000+     & Apr 14, 2019  & 1.1.1   & 8       & 349        \\ \hline
	EP Mobile               & Medical                   & 50,000+     & Aug 25, 2011  & 2.22    & 65      & 775        \\ \hline
	Fast                    & Tools                     & 50,000+     & Jan 15, 2013  & 6.7     & 37      & 506        \\ \hline
	Gadgetbridge            & Tools                     & 500,000+    & Jan 4, 2015   & 0.41.0  & 189     & 6544       \\ \hline
	Gnucash                 & Finance                   & 100,000+    & May 13, 2012  & 2.0.5   & 117     & 1730       \\ \hline
	Kdeconnect              & Productivity              & 500,000+    & Jun 2, 2013   & 1.13.2  & 72      & 2568       \\ \hline
	Kouchat                 & Communication             & 5,000+      & Nov 13, 2011  & 1.1.1   & 17      & 1197       \\ \hline
	LaunchTime              & Personalization           & 500+        & Jan 21, 2017  & 0.8.5   & 25      & 1007       \\ \hline
	Loyalty Card Keychain   & Shopping                  & 10,000+     & Jan 30, 2016  & 0.26.1  & 39      & 628        \\ \hline
	Materialistic           & News and Magazines        & 100,000+    & Jan 18, 2015  & 3.3.0   & 67      & 1731       \\ \hline
	Mi Manga Nu             & Comics                    & -           & May 24, 2015  & 1.121   & 93      & 1877       \\ \hline
	NewPipe                 & Video Players and Editors & 1,000,000+  & Sep 13, 2015  & 0.17.3  & 102     & 8461       \\ \hline
	NewPipe-Legacy          & Video Players and Editors & 100,000+    & Sep 13, 2015  & 0.18.1  & 78      & 8169       \\ \hline
	Omni Notes              & Productivity              & 100,000+    & Oct 27, 2013  & 5.5.2   & 127     & 3138       \\ \hline
	OpenFoodFacts           & Health \& Fitness         & 500,000+    & May 3, 2015   & 3.2.5   & 64      & 7583       \\ \hline
	OpenScale               & Health \& Fitness         & 1,000+      & Dec 7, 2014   & 2.2.0   & 46      & 1977       \\ \hline
	PasseGares              & Travel \& Local           & -           & Nov 26, 2016  & 1.4.0   & 34      & 669        \\ \hline
	Piwigo                  & Photography               & 1,000+      & Dec 15, 2018  & 1.0.2   & 5       & 584        \\ \hline
	Pedometer               & Health \& Fitness         & 10,000+     & Mar 18, 2018  & 1.0.5   & 5       & 487        \\ \hline
	Slide                   & Personalization           & -           & Sep 27, 2015  & 6.2.2   & 168     & 4060       \\ \hline
	Telecine                & Entertainment             & 50,000+     & Oct 25, 2014  & 3.1.20  & 17      & 264        \\ \hline
	Unit Converter Ultimate & Tools                     & 1,000,000+  & Aug 19, 2015  & 5.6.0   & 20      & 420        \\ \hline
	Wikipedia               & Books and Reference       & 10,000,000+ & Oct 20, 2013  & 2.7.5   & 221     & 17076      \\ \hline
\end{tabular}}
\end{table*}

==> tables/deprecated.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
	\caption{Deprecated APIs is Android API Evaluation.}
	\label{tab:num_deprecated}
	\centering
	\begin{tabular}{|c|c|cc|cc|}
		\hline
		\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}API\\ Level\end{tabular}} & \multirow{2}{*}{Release Date} & \multicolumn{2}{c|}{Fields}        & \multicolumn{2}{c|}{Methods}        \\ \cline{3-6} 
		&                               & \multicolumn{1}{c|}{New} & Removed & \multicolumn{1}{c|}{New}  & Removed \\ \hline
		20                                                                   & June 25, 2014                 & \multicolumn{1}{c|}{2}   & 0       & \multicolumn{1}{c|}{5}    & 1       \\ \hline
		21                                                                   & November 12, 2014             & \multicolumn{1}{c|}{75}  & 2       & \multicolumn{1}{c|}{117}  & 29      \\ \hline
		22                                                                   & March 9, 2015                 & \multicolumn{1}{c|}{1}   & 13      & \multicolumn{1}{c|}{128}  & 3       \\ \hline
		23                                                                   & October 5, 2015               & \multicolumn{1}{c|}{89}  & 83      & \multicolumn{1}{c|}{132}  & 38      \\ \hline
		24                                                                   & August 22, 2016               & \multicolumn{1}{c|}{31}  & 5       & \multicolumn{1}{c|}{127}  & 13      \\ \hline
		25                                                                   & October 4, 2016               & \multicolumn{1}{c|}{0}   & 0       & \multicolumn{1}{c|}{1}    & 0       \\ \hline
		26                                                                   & August 21, 2017               & \multicolumn{1}{c|}{69}  & 0       & \multicolumn{1}{c|}{139}  & 18      \\ \hline
		27                                                                   & December 5, 2017              & \multicolumn{1}{c|}{2}   & 0       & \multicolumn{1}{c|}{176}  & 16      \\ \hline
		28                                                                   & August 6, 2018                & \multicolumn{1}{c|}{272} & 8       & \multicolumn{1}{c|}{673}  & 169     \\ \hline
		29                                                                   & September 3, 2019             & \multicolumn{1}{c|}{503} & 12      & \multicolumn{1}{c|}{1443} & 14      \\ \hline
		30                                                                   & September 8, 2020             & \multicolumn{1}{c|}{128} & 8       & \multicolumn{1}{c|}{295}  & 0       \\ \hline
		31                                                                   & July 6, 2021                  & \multicolumn{1}{c|}{231} & 2       & \multicolumn{1}{c|}{896}  & 3       \\ \hline
		32                                                                   & December 6, 2021              & \multicolumn{1}{c|}{1}   & 0       & \multicolumn{1}{c|}{2}    & 0       \\ \hline
		33                                                                   & June 3, 2022                  & \multicolumn{1}{c|}{47}  & 0       & \multicolumn{1}{c|}{230}  & 7       \\ \hline
	\end{tabular}
\end{table}

==> tables/stackoverlow.tex <==
\begin{table*}
	\caption{Stack overflow API and parameters used to collect related posts}
	\label{tab:stackoverflow}
	\centering
	\scalebox{0.80}{
	\begin{tabular}{|l|c|c|c|}
		\hline
		Task              & API                      & Parameter   & Return                        \\ \hline
		Search query         & (GET) /search/advanced           & query, tag, site & A list of questions with question ids \\ \hline
		Get question body & (GET) /questions/\{id\} & question id & Question for the provided id \\ \hline
		Get question answers & (GET) /questions/\{ids\}/answers & question id      & A list of answers with the answer ids \\ \hline
		Get answers body  & (GET) /answers/\{id\}   & answer id   & Answer for the provided id  \\ \hline
	\end{tabular}}
\end{table*}
